Premise Recovery in Software Design: What Does This Decision Rest On?

Design decisions shape software architecture, and writing them down preserves the reasons behind it. Architecture decision records (ADRs) capture them, each with its context, choice, and consequences. A decision can depend on earlier ones: reversing one of them would force its review. We call these its premises. Yet ADRs do not always name their premises. When a decision is reversed, engineers supersede its ADR and search by hand for what it affects. That search can miss ADRs resting on an unnamed premise. We frame this as premise recovery: given an ADR with identifiers masked, find its premises among earlier records. We collect 1,060 ADRs from 36 repositories and label 1,529 candidate pairs for 60 target ADRs. Two LLM annotators agree at \k{appa} = 0.859. An independent human annotator, blind to their labels, agrees with the stated/implicit tag on 30 of 32 premises (\k{appa} = 0.875). We compare 7 open-weight models with 2 baselines that use no LLM. Qwen3.8-27B reaches F1 0.756, against 0.466 for word overlap; 2 models added post hoc score similarly. On the 11 premises whose titles barely overlap the target, it finds 0.758, while word overlap finds none. Reasoning raises its recall of implicit premises but not its F1. Word overlap with as many predictions gains 69% as much. We find only 2 to 3 stale dependents, though we searched for unlinked ones in only 30 of 66 supersessions. Open models could thus suggest unwritten premises when a decision is reversed, with precision between 0.68 and 0.78.

==> tables/numbers.tex <==
% Generated by code/make_tables.py from analysis.json and budget_matched.json; do not edit by hand.
\makeatletter
\newcommand{\res}[2]{\@ifundefined{r@#1@#2}{\textbf{??}}{\@nameuse{r@#1@#2}}}
\@namedef{r@BGE@AdjMax}{0.478}
\@namedef{r@BGE@AdjMin}{0.378}
\@namedef{r@BGE@F1}{0.435}
\@namedef{r@BGE@Fadjudicated}{0.420}
\@namedef{r@BGE@Fhi}{0.541}
\@namedef{r@BGE@Flenient}{0.432}
\@namedef{r@BGE@Flinked}{0.500}
\@namedef{r@BGE@Flo}{0.322}
\@namedef{r@BGE@Fmain}{0.435}
\@namedef{r@BGE@Fnolink}{0.214}
\@namedef{r@BGE@Fnopred}{0.410}
\@namedef{r@BGE@Fsilver}{0.456}
\@namedef{r@BGE@Fstrict}{0.419}
\@namedef{r@BGE@P}{0.429}
\@namedef{r@BGE@Pred}{1.05}
\@namedef{r@BGE@R}{0.443}
\@namedef{r@BGE@Rhigh}{0.520}
\@namedef{r@BGE@Rim}{0.125}
\@namedef{r@BGE@Rimadjudicated}{0.143}
\@namedef{r@BGE@Rimlenient}{0.125}
\@namedef{r@BGE@Rimlo}{0.000}
\@namedef{r@BGE@Rimmain}{0.125}
\@namedef{r@BGE@Rimnopred}{0.125}
\@namedef{r@BGE@Rimsilver}{0.000}
\@namedef{r@BGE@Rimstrict}{0.125}
\@namedef{r@BGE@Rlow}{0.091}
\@namedef{r@BGE@RlowHi}{0.400}
\@namedef{r@BGE@RlowLo}{0.000}
\@namedef{r@BGE@Rlown}{1.0}
\@namedef{r@BGE@Rst}{0.548}
\@namedef{r@BGE@Seeds}{1}
\@namedef{r@ET@AdjMax}{0.621}
\@namedef{r@ET@AdjMin}{0.510}
\@namedef{r@ET@F1}{0.586}
\@namedef{r@ET@Fadjudicated}{0.566}
\@namedef{r@ET@Fhi}{0.682}
\@namedef{r@ET@Flenient}{0.568}
\@namedef{r@ET@Flinked}{0.704}
\@namedef{r@ET@Flo}{0.488}
\@namedef{r@ET@Fmain}{0.586}
\@namedef{r@ET@Fnolink}{0.254}
\@namedef{r@ET@Fnopred}{0.558}
\@namedef{r@ET@Fsilver}{0.563}
\@namedef{r@ET@Fstrict}{0.560}
\@namedef{r@ET@P}{0.557}
\@namedef{r@ET@Pred}{1.13}
\@namedef{r@ET@R}{0.617}
\@namedef{r@ET@Rhigh}{0.707}
\@namedef{r@ET@Rim}{0.229}
\@namedef{r@ET@Rimadjudicated}{0.317}
\@namedef{r@ET@Rimlenient}{0.229}
\@namedef{r@ET@Rimlo}{0.048}
\@namedef{r@ET@Rimmain}{0.229}
\@namedef{r@ET@Rimnopred}{0.229}
\@namedef{r@ET@Rimsilver}{0.000}
\@namedef{r@ET@Rimstrict}{0.229}
\@namedef{r@ET@Rlow}{0.212}
\@namedef{r@ET@RlowHi}{0.533}
\@namedef{r@ET@RlowLo}{0.000}
\@namedef{r@ET@Rlown}{2.3}
\@namedef{r@ET@Rst}{0.770}
\@namedef{r@ET@Seeds}{3}
\@namedef{r@ET@bmlexF1}{0.412}
\@namedef{r@ET@bmlexRim}{0.312}
\@namedef{r@ET@bmpred}{1.23}
\@namedef{r@ETD@AdjMax}{0.495}
\@namedef{r@ETD@AdjMin}{0.408}
\@namedef{r@ETD@F1}{0.458}
\@namedef{r@ETD@Fadjudicated}{0.454}
\@namedef{r@ETD@Fhi}{0.603}
\@namedef{r@ETD@Flenient}{0.458}
\@namedef{r@ETD@Flinked}{0.505}
\@namedef{r@ETD@Flo}{0.339}
\@namedef{r@ETD@Fmain}{0.458}
\@namedef{r@ETD@Fnolink}{0.328}
\@namedef{r@ETD@Fnopred}{0.429}
\@namedef{r@ETD@Fsilver}{0.381}
\@namedef{r@ETD@Fstrict}{0.442}
\@namedef{r@ETD@P}{0.381}
\@namedef{r@ETD@Pred}{1.57}
\@namedef{r@ETD@R}{0.579}
\@namedef{r@ETD@Rhigh}{0.667}
\@namedef{r@ETD@Rim}{0.292}
\@namedef{r@ETD@Rimadjudicated}{0.317}
\@namedef{r@ETD@Rimlenient}{0.292}
\@namedef{r@ETD@Rimlo}{0.000}
\@namedef{r@ETD@Rimmain}{0.292}
\@namedef{r@ETD@Rimnopred}{0.292}
\@namedef{r@ETD@Rimsilver}{0.000}
\@namedef{r@ETD@Rimstrict}{0.292}
\@namedef{r@ETD@Rlow}{0.182}
\@namedef{r@ETD@RlowHi}{0.500}
\@namedef{r@ETD@RlowLo}{0.000}
\@namedef{r@ETD@Rlown}{2.0}
\@namedef{r@ETD@Rst}{0.683}
\@namedef{r@ETD@Seeds}{3}
\@namedef{r@ETD@bmlexF1}{0.360}
\@namedef{r@ETD@bmlexRim}{0.312}
\@namedef{r@ETD@bmpred}{1.66}
\@namedef{r@GTDR@AdjMax}{0.657}
\@namedef{r@GTDR@AdjMin}{0.559}
\@namedef{r@GTDR@F1}{0.624}
\@namedef{r@GTDR@Fadjudicated}{0.609}
\@namedef{r@GTDR@Fhi}{0.721}
\@namedef{r@GTDR@Flenient}{0.620}
\@namedef{r@GTDR@Flinked}{0.654}
\@namedef{r@GTDR@Flo}{0.533}
\@namedef{r@GTDR@Fmain}{0.624}
\@namedef{r@GTDR@Fnolink}{0.522}
\@namedef{r@GTDR@Fnopred}{0.605}
\@namedef{r@GTDR@Fsilver}{0.435}
\@namedef{r@GTDR@Fstrict}{0.595}
\@namedef{r@GTDR@P}{0.499}
\@namedef{r@GTDR@Pred}{1.71}
\@namedef{r@GTDR@R}{0.836}
\@namedef{r@GTDR@Rhigh}{0.833}
\@namedef{r@GTDR@Rim}{0.729}
\@namedef{r@GTDR@Rimadjudicated}{0.667}
\@namedef{r@GTDR@Rimlenient}{0.729}
\@namedef{r@GTDR@Rimlo}{0.762}
\@namedef{r@GTDR@Rimmain}{0.729}
\@namedef{r@GTDR@Rimnopred}{0.729}
\@namedef{r@GTDR@Rimsilver}{0.000}
\@namedef{r@GTDR@Rimstrict}{0.729}
\@namedef{r@GTDR@Rlow}{0.848}
\@namedef{r@GTDR@RlowHi}{1.000}
\@namedef{r@GTDR@RlowLo}{0.600}
\@namedef{r@GTDR@Rlown}{9.3}
\@namedef{r@GTDR@Rst}{0.865}
\@namedef{r@GTDR@Seeds}{3}
\@namedef{r@GTDR@bmlexF1}{0.509}
\@namedef{r@GTDR@bmlexRim}{0.521}
\@namedef{r@GTDR@bmpred}{1.85}
\@namedef{r@GTR@AdjMax}{0.581}
\@namedef{r@GTR@AdjMin}{0.496}
\@namedef{r@GTR@F1}{0.547}
\@namedef{r@GTR@Fadjudicated}{0.536}
\@namedef{r@GTR@Fhi}{0.636}
\@namedef{r@GTR@Flenient}{0.549}
\@namedef{r@GTR@Flinked}{0.618}
\@namedef{r@GTR@Flo}{0.468}
\@namedef{r@GTR@Fmain}{0.547}
\@namedef{r@GTR@Fnolink}{0.335}
\@namedef{r@GTR@Fnopred}{0.527}
\@namedef{r@GTR@Fsilver}{0.419}
\@namedef{r@GTR@Fstrict}{0.526}
\@namedef{r@GTR@P}{0.411}
\@namedef{r@GTR@Pred}{2.03}
\@namedef{r@GTR@R}{0.820}
\@namedef{r@GTR@Rhigh}{0.853}
\@namedef{r@GTR@Rim}{0.667}
\@namedef{r@GTR@Rimadjudicated}{0.635}
\@namedef{r@GTR@Rimlenient}{0.667}
\@namedef{r@GTR@Rimlo}{0.667}
\@namedef{r@GTR@Rimmain}{0.667}
\@namedef{r@GTR@Rimnopred}{0.667}
\@namedef{r@GTR@Rimsilver}{0.000}
\@namedef{r@GTR@Rimstrict}{0.667}
\@namedef{r@GTR@Rlow}{0.667}
\@namedef{r@GTR@RlowHi}{1.000}
\@namedef{r@GTR@RlowLo}{0.462}
\@namedef{r@GTR@Rlown}{7.3}
\@namedef{r@GTR@Rst}{0.881}
\@namedef{r@GTR@Seeds}{3}
\@namedef{r@GTR@bmlexF1}{0.474}
\@namedef{r@GTR@bmlexRim}{0.500}
\@namedef{r@GTR@bmpred}{2.17}
\@namedef{r@LEX@AdjMax}{0.508}
\@namedef{r@LEX@AdjMin}{0.400}
\@namedef{r@LEX@F1}{0.466}
\@namedef{r@LEX@Fadjudicated}{0.431}
\@namedef{r@LEX@Fhi}{0.589}
\@namedef{r@LEX@Flenient}{0.457}
\@namedef{r@LEX@Flinked}{0.515}
\@namedef{r@LEX@Flo}{0.326}
\@namedef{r@LEX@Fmain}{0.466}
\@namedef{r@LEX@Fnolink}{0.133}
\@namedef{r@LEX@Fnopred}{0.455}
\@namedef{r@LEX@Fsilver}{0.528}
\@namedef{r@LEX@Fstrict}{0.446}
\@namedef{r@LEX@P}{0.491}
\@namedef{r@LEX@Pred}{0.92}
\@namedef{r@LEX@R}{0.443}
\@namedef{r@LEX@Rhigh}{0.540}
\@namedef{r@LEX@Rim}{0.125}
\@namedef{r@LEX@Rimadjudicated}{0.143}
\@namedef{r@LEX@Rimlenient}{0.125}
\@namedef{r@LEX@Rimlo}{0.000}
\@namedef{r@LEX@Rimmain}{0.125}
\@namedef{r@LEX@Rimnopred}{0.125}
\@namedef{r@LEX@Rimsilver}{0.000}
\@namedef{r@LEX@Rimstrict}{0.125}
\@namedef{r@LEX@Rlow}{0.000}
\@namedef{r@LEX@RlowHi}{0.000}
\@namedef{r@LEX@RlowLo}{0.000}
\@namedef{r@LEX@Rlown}{0.0}
\@namedef{r@LEX@Rst}{0.571}
\@namedef{r@LEX@Seeds}{1}
\@namedef{r@LEX@rankmain}{15}
\@namedef{r@LEX@rankmainord}{fifteenth}
\@namedef{r@LEX@ranksilver}{8}
\@namedef{r@LEX@ranksilverord}{eighth}
\@namedef{r@LT@AdjMax}{0.276}
\@namedef{r@LT@AdjMin}{0.230}
\@namedef{r@LT@F1}{0.243}
\@namedef{r@LT@Fadjudicated}{0.253}
\@namedef{r@LT@Fhi}{0.347}
\@namedef{r@LT@Flenient}{0.266}
\@namedef{r@LT@Flinked}{0.296}
\@namedef{r@LT@Flo}{0.165}
\@namedef{r@LT@Fmain}{0.243}
\@namedef{r@LT@Fnolink}{0.135}
\@namedef{r@LT@Fnopred}{0.232}
\@namedef{r@LT@Fsilver}{0.181}
\@namedef{r@LT@Fstrict}{0.238}
\@namedef{r@LT@P}{0.150}
\@namedef{r@LT@Pred}{4.51}
\@namedef{r@LT@R}{0.656}
\@namedef{r@LT@Rhigh}{0.660}
\@namedef{r@LT@Rim}{0.583}
\@namedef{r@LT@Rimadjudicated}{0.540}
\@namedef{r@LT@Rimlenient}{0.583}
\@namedef{r@LT@Rimlo}{0.619}
\@namedef{r@LT@Rimmain}{0.583}
\@namedef{r@LT@Rimnopred}{0.583}
\@namedef{r@LT@Rimsilver}{0.000}
\@namedef{r@LT@Rimstrict}{0.583}
\@namedef{r@LT@Rlow}{0.636}
\@namedef{r@LT@RlowHi}{0.944}
\@namedef{r@LT@RlowLo}{0.438}
\@namedef{r@LT@Rlown}{7.0}
\@namedef{r@LT@Rst}{0.698}
\@namedef{r@LT@Seeds}{3}
\@namedef{r@LT@bmlexF1}{0.269}
\@namedef{r@LT@bmlexRim}{0.604}
\@namedef{r@LT@bmpred}{4.63}
\@namedef{r@LTD@AdjMax}{0.195}
\@namedef{r@LTD@AdjMin}{0.157}
\@namedef{r@LTD@F1}{0.163}
\@namedef{r@LTD@Fadjudicated}{0.178}
\@namedef{r@LTD@Fhi}{0.263}
\@namedef{r@LTD@Flenient}{0.192}
\@namedef{r@LTD@Flinked}{0.184}
\@namedef{r@LTD@Flo}{0.102}
\@namedef{r@LTD@Fmain}{0.163}
\@namedef{r@LTD@Fnolink}{0.104}
\@namedef{r@LTD@Fnopred}{0.153}
\@namedef{r@LTD@Fsilver}{0.119}
\@namedef{r@LTD@Fstrict}{0.159}
\@namedef{r@LTD@P}{0.091}
\@namedef{r@LTD@Pred}{8.52}
\@namedef{r@LTD@R}{0.749}
\@namedef{r@LTD@Rhigh}{0.773}
\@namedef{r@LTD@Rim}{0.750}
\@namedef{r@LTD@Rimadjudicated}{0.730}
\@namedef{r@LTD@Rimlenient}{0.750}
\@namedef{r@LTD@Rimlo}{0.667}
\@namedef{r@LTD@Rimmain}{0.750}
\@namedef{r@LTD@Rimnopred}{0.750}
\@namedef{r@LTD@Rimsilver}{0.000}
\@namedef{r@LTD@Rimstrict}{0.750}
\@namedef{r@LTD@Rlow}{0.636}
\@namedef{r@LTD@RlowHi}{0.905}
\@namedef{r@LTD@RlowLo}{0.400}
\@namedef{r@LTD@Rlown}{7.0}
\@namedef{r@LTD@Rst}{0.770}
\@namedef{r@LTD@Seeds}{3}
\@namedef{r@LTD@bmlexF1}{0.186}
\@namedef{r@LTD@bmlexRim}{0.792}
\@namedef{r@LTD@bmpred}{8.76}
\@namedef{r@MT@AdjMax}{0.742}
\@namedef{r@MT@AdjMin}{0.606}
\@namedef{r@MT@F1}{0.708}
\@namedef{r@MT@Fadjudicated}{0.644}
\@namedef{r@MT@Fhi}{0.806}
\@namedef{r@MT@Flenient}{0.679}
\@namedef{r@MT@Flinked}{0.736}
\@namedef{r@MT@Flo}{0.589}
\@namedef{r@MT@Fmain}{0.708}
\@namedef{r@MT@Fnolink}{0.596}
\@namedef{r@MT@Fnopred}{0.686}
\@namedef{r@MT@Fsilver}{0.633}
\@namedef{r@MT@Fstrict}{0.665}
\@namedef{r@MT@P}{0.778}
\@namedef{r@MT@Pred}{0.85}
\@namedef{r@MT@R}{0.650}
\@namedef{r@MT@Rhigh}{0.693}
\@namedef{r@MT@Rim}{0.229}
\@namedef{r@MT@Rimadjudicated}{0.254}
\@namedef{r@MT@Rimlenient}{0.229}
\@namedef{r@MT@Rimlo}{0.143}
\@namedef{r@MT@Rimmain}{0.229}
\@namedef{r@MT@Rimnopred}{0.229}
\@namedef{r@MT@Rimsilver}{0.000}
\@namedef{r@MT@Rimstrict}{0.229}
\@namedef{r@MT@Rlow}{0.455}
\@namedef{r@MT@RlowHi}{0.833}
\@namedef{r@MT@RlowLo}{0.111}
\@namedef{r@MT@Rlown}{5.0}
\@namedef{r@MT@Rst}{0.810}
\@namedef{r@MT@Seeds}{3}
\@namedef{r@MTD@AdjMax}{0.782}
\@namedef{r@MTD@AdjMin}{0.649}
\@namedef{r@MTD@F1}{0.754}
\@namedef{r@MTD@Fadjudicated}{0.702}
\@namedef{r@MTD@Fhi}{0.851}
\@namedef{r@MTD@Flenient}{0.718}
\@namedef{r@MTD@Flinked}{0.765}
\@namedef{r@MTD@Flo}{0.652}
\@namedef{r@MTD@Fmain}{0.754}
\@namedef{r@MTD@Fnolink}{0.715}
\@namedef{r@MTD@Fnopred}{0.736}
\@namedef{r@MTD@Fsilver}{0.593}
\@namedef{r@MTD@Fstrict}{0.710}
\@namedef{r@MTD@P}{0.791}
\@namedef{r@MTD@Pred}{0.93}
\@namedef{r@MTD@R}{0.721}
\@namedef{r@MTD@Rhigh}{0.753}
\@namedef{r@MTD@Rim}{0.417}
\@namedef{r@MTD@Rimadjudicated}{0.444}
\@namedef{r@MTD@Rimlenient}{0.417}
\@namedef{r@MTD@Rimlo}{0.333}
\@namedef{r@MTD@Rimmain}{0.417}
\@namedef{r@MTD@Rimnopred}{0.417}
\@namedef{r@MTD@Rimsilver}{0.000}
\@namedef{r@MTD@Rimstrict}{0.417}
\@namedef{r@MTD@Rlow}{0.576}
\@namedef{r@MTD@RlowHi}{1.000}
\@namedef{r@MTD@RlowLo}{0.190}
\@namedef{r@MTD@Rlown}{6.3}
\@namedef{r@MTD@Rst}{0.817}
\@namedef{r@MTD@Seeds}{3}
\@namedef{r@MTDR@AdjMax}{0.816}
\@namedef{r@MTDR@AdjMin}{0.690}
\@namedef{r@MTDR@F1}{0.796}
\@namedef{r@MTDR@Fadjudicated}{0.740}
\@namedef{r@MTDR@Fhi}{0.868}
\@namedef{r@MTDR@Flenient}{0.748}
\@namedef{r@MTDR@Flinked}{0.825}
\@namedef{r@MTDR@Flo}{0.721}
\@namedef{r@MTDR@Fmain}{0.796}
\@namedef{r@MTDR@Fnolink}{0.676}
\@namedef{r@MTDR@Fnopred}{0.782}
\@namedef{r@MTDR@Fsilver}{0.623}
\@namedef{r@MTDR@Fstrict}{0.755}
\@namedef{r@MTDR@P}{0.783}
\@namedef{r@MTDR@Pred}{1.05}
\@namedef{r@MTDR@R}{0.809}
\@namedef{r@MTDR@Rhigh}{0.840}
\@namedef{r@MTDR@Rim}{0.667}
\@namedef{r@MTDR@Rimadjudicated}{0.619}
\@namedef{r@MTDR@Rimlenient}{0.667}
\@namedef{r@MTDR@Rimlo}{0.571}
\@namedef{r@MTDR@Rimmain}{0.667}
\@namedef{r@MTDR@Rimnopred}{0.667}
\@namedef{r@MTDR@Rimsilver}{0.000}
\@namedef{r@MTDR@Rimstrict}{0.667}
\@namedef{r@MTDR@Rlow}{0.667}
\@namedef{r@MTDR@RlowHi}{1.000}
\@namedef{r@MTDR@RlowLo}{0.429}
\@namedef{r@MTDR@Rlown}{7.3}
\@namedef{r@MTDR@Rst}{0.849}
\@namedef{r@MTDR@Seeds}{3}
\@namedef{r@MTR@AdjMax}{0.806}
\@namedef{r@MTR@AdjMin}{0.678}
\@namedef{r@MTR@F1}{0.787}
\@namedef{r@MTR@Fadjudicated}{0.725}
\@namedef{r@MTR@Fhi}{0.870}
\@namedef{r@MTR@Flenient}{0.731}
\@namedef{r@MTR@Flinked}{0.801}
\@namedef{r@MTR@Flo}{0.711}
\@namedef{r@MTR@Fmain}{0.787}
\@namedef{r@MTR@Fnolink}{0.732}
\@namedef{r@MTR@Fnopred}{0.772}
\@namedef{r@MTR@Fsilver}{0.646}
\@namedef{r@MTR@Fstrict}{0.751}
\@namedef{r@MTR@P}{0.818}
\@namedef{r@MTR@Pred}{0.94}
\@namedef{r@MTR@R}{0.760}
\@namedef{r@MTR@Rhigh}{0.807}
\@namedef{r@MTR@Rim}{0.583}
\@namedef{r@MTR@Rimadjudicated}{0.524}
\@namedef{r@MTR@Rimlenient}{0.583}
\@namedef{r@MTR@Rimlo}{0.333}
\@namedef{r@MTR@Rimmain}{0.583}
\@namedef{r@MTR@Rimnopred}{0.583}
\@namedef{r@MTR@Rimsilver}{0.000}
\@namedef{r@MTR@Rimstrict}{0.583}
\@namedef{r@MTR@Rlow}{0.545}
\@namedef{r@MTR@RlowHi}{0.944}
\@namedef{r@MTR@RlowLo}{0.222}
\@namedef{r@MTR@Rlown}{6.0}
\@namedef{r@MTR@Rst}{0.849}
\@namedef{r@MTR@Seeds}{3}
\@namedef{r@QT@AdjMax}{0.731}
\@namedef{r@QT@AdjMin}{0.615}
\@namedef{r@QT@F1}{0.706}
\@namedef{r@QT@Fadjudicated}{0.674}
\@namedef{r@QT@Fhi}{0.807}
\@namedef{r@QT@Flenient}{0.669}
\@namedef{r@QT@Flinked}{0.734}
\@namedef{r@QT@Flo}{0.603}
\@namedef{r@QT@Fmain}{0.706}
\@namedef{r@QT@Fnolink}{0.579}
\@namedef{r@QT@Fnopred}{0.697}
\@namedef{r@QT@Fsilver}{0.519}
\@namedef{r@QT@Fstrict}{0.674}
\@namedef{r@QT@P}{0.674}
\@namedef{r@QT@Pred}{1.12}
\@namedef{r@QT@R}{0.743}
\@namedef{r@QT@Rhigh}{0.787}
\@namedef{r@QT@Rim}{0.667}
\@namedef{r@QT@Rimadjudicated}{0.619}
\@namedef{r@QT@Rimlenient}{0.667}
\@namedef{r@QT@Rimlo}{0.524}
\@namedef{r@QT@Rimmain}{0.667}
\@namedef{r@QT@Rimnopred}{0.667}
\@namedef{r@QT@Rimsilver}{0.000}
\@namedef{r@QT@Rimstrict}{0.667}
\@namedef{r@QT@Rlow}{0.545}
\@namedef{r@QT@RlowHi}{0.944}
\@namedef{r@QT@RlowLo}{0.231}
\@namedef{r@QT@Rlown}{6.0}
\@namedef{r@QT@Rst}{0.770}
\@namedef{r@QT@Seeds}{3}
\@namedef{r@QT@bmlexF1}{0.509}
\@namedef{r@QT@bmlexRim}{0.333}
\@namedef{r@QT@bmpred}{1.24}
\@namedef{r@QTD@AdjMax}{0.793}
\@namedef{r@QTD@AdjMin}{0.664}
\@namedef{r@QTD@F1}{0.756}
\@namedef{r@QTD@Fadjudicated}{0.719}
\@namedef{r@QTD@Fhi}{0.812}
\@namedef{r@QTD@Flenient}{0.759}
\@namedef{r@QTD@Flinked}{0.788}
\@namedef{r@QTD@Flo}{0.697}
\@namedef{r@QTD@Fmain}{0.756}
\@namedef{r@QTD@Fnolink}{0.614}
\@namedef{r@QTD@Fnopred}{0.741}
\@namedef{r@QTD@Fsilver}{0.563}
\@namedef{r@QTD@Fstrict}{0.695}
\@namedef{r@QTD@P}{0.683}
\@namedef{r@QTD@Pred}{1.26}
\@namedef{r@QTD@R}{0.847}
\@namedef{r@QTD@Rhigh}{0.867}
\@namedef{r@QTD@Rim}{0.667}
\@namedef{r@QTD@Rimadjudicated}{0.635}
\@namedef{r@QTD@Rimlenient}{0.667}
\@namedef{r@QTD@Rimlo}{0.667}
\@namedef{r@QTD@Rimmain}{0.667}
\@namedef{r@QTD@Rimnopred}{0.667}
\@namedef{r@QTD@Rimsilver}{0.000}
\@namedef{r@QTD@Rimstrict}{0.667}
\@namedef{r@QTD@Rlow}{0.758}
\@namedef{r@QTD@RlowHi}{1.000}
\@namedef{r@QTD@RlowLo}{0.500}
\@namedef{r@QTD@Rlown}{8.3}
\@namedef{r@QTD@Rst}{0.929}
\@namedef{r@QTD@Seeds}{3}
\@namedef{r@QTD@bmlexF1}{0.511}
\@namedef{r@QTD@bmlexRim}{0.333}
\@namedef{r@QTD@bmpred}{1.47}
\@namedef{r@QTDR@AdjMax}{0.791}
\@namedef{r@QTDR@AdjMin}{0.668}
\@namedef{r@QTDR@F1}{0.750}
\@namedef{r@QTDR@Fadjudicated}{0.734}
\@namedef{r@QTDR@Fhi}{0.847}
\@namedef{r@QTDR@Flenient}{0.776}
\@namedef{r@QTDR@Flinked}{0.797}
\@namedef{r@QTDR@Flo}{0.661}
\@namedef{r@QTDR@Fmain}{0.750}
\@namedef{r@QTDR@Fnolink}{0.591}
\@namedef{r@QTDR@Fnopred}{0.737}
\@namedef{r@QTDR@Fsilver}{0.516}
\@namedef{r@QTDR@Fstrict}{0.682}
\@namedef{r@QTDR@P}{0.620}
\@namedef{r@QTDR@Pred}{1.56}
\@namedef{r@QTDR@R}{0.951}
\@namedef{r@QTDR@Rhigh}{0.960}
\@namedef{r@QTDR@Rim}{0.938}
\@namedef{r@QTDR@Rimadjudicated}{0.937}
\@namedef{r@QTDR@Rimlenient}{0.938}
\@namedef{r@QTDR@Rimlo}{0.857}
\@namedef{r@QTDR@Rimmain}{0.938}
\@namedef{r@QTDR@Rimnopred}{0.938}
\@namedef{r@QTDR@Rimsilver}{0.000}
\@namedef{r@QTDR@Rimstrict}{0.938}
\@namedef{r@QTDR@Rlow}{0.909}
\@namedef{r@QTDR@RlowHi}{1.000}
\@namedef{r@QTDR@RlowLo}{0.769}
\@namedef{r@QTDR@Rlown}{10.0}
\@namedef{r@QTDR@Rst}{0.952}
\@namedef{r@QTDR@Seeds}{3}
\@namedef{r@QTDR@bmlexF1}{0.502}
\@namedef{r@QTDR@bmlexRim}{0.521}
\@namedef{r@QTDR@bmpred}{1.82}
\@namedef{r@QTR@AdjMax}{0.708}
\@namedef{r@QTR@AdjMin}{0.600}
\@namedef{r@QTR@F1}{0.666}
\@namedef{r@QTR@Fadjudicated}{0.660}
\@namedef{r@QTR@Fhi}{0.763}
\@namedef{r@QTR@Flenient}{0.686}
\@namedef{r@QTR@Flinked}{0.720}
\@namedef{r@QTR@Flo}{0.585}
\@namedef{r@QTR@Fmain}{0.666}
\@namedef{r@QTR@Fnolink}{0.488}
\@namedef{r@QTR@Fnopred}{0.652}
\@namedef{r@QTR@Fsilver}{0.460}
\@namedef{r@QTR@Fstrict}{0.620}
\@namedef{r@QTR@P}{0.514}
\@namedef{r@QTR@Pred}{1.87}
\@namedef{r@QTR@R}{0.945}
\@namedef{r@QTR@Rhigh}{0.967}
\@namedef{r@QTR@Rim}{0.875}
\@namedef{r@QTR@Rimadjudicated}{0.889}
\@namedef{r@QTR@Rimlenient}{0.875}
\@namedef{r@QTR@Rimlo}{0.762}
\@namedef{r@QTR@Rimmain}{0.875}
\@namedef{r@QTR@Rimnopred}{0.875}
\@namedef{r@QTR@Rimsilver}{0.000}
\@namedef{r@QTR@Rimstrict}{0.875}
\@namedef{r@QTR@Rlow}{0.848}
\@namedef{r@QTR@RlowHi}{1.000}
\@namedef{r@QTR@RlowLo}{0.583}
\@namedef{r@QTR@Rlown}{9.3}
\@namedef{r@QTR@Rst}{0.968}
\@namedef{r@QTR@Seeds}{3}
\@namedef{r@QTR@bmlexF1}{0.510}
\@namedef{r@QTR@bmlexRim}{0.521}
\@namedef{r@QTR@bmpred}{2.10}
\@namedef{r@WT@AdjMax}{0.495}
\@namedef{r@WT@AdjMin}{0.410}
\@namedef{r@WT@F1}{0.473}
\@namedef{r@WT@Fadjudicated}{0.452}
\@namedef{r@WT@Fhi}{0.571}
\@namedef{r@WT@Flenient}{0.439}
\@namedef{r@WT@Flinked}{0.546}
\@namedef{r@WT@Flo}{0.379}
\@namedef{r@WT@Fmain}{0.473}
\@namedef{r@WT@Fnolink}{0.220}
\@namedef{r@WT@Fnopred}{0.481}
\@namedef{r@WT@Fsilver}{0.393}
\@namedef{r@WT@Fstrict}{0.463}
\@namedef{r@WT@P}{0.471}
\@namedef{r@WT@Pred}{1.03}
\@namedef{r@WT@R}{0.475}
\@namedef{r@WT@Rhigh}{0.533}
\@namedef{r@WT@Rim}{0.333}
\@namedef{r@WT@Rimadjudicated}{0.302}
\@namedef{r@WT@Rimlenient}{0.333}
\@namedef{r@WT@Rimlo}{0.286}
\@namedef{r@WT@Rimmain}{0.333}
\@namedef{r@WT@Rimnopred}{0.333}
\@namedef{r@WT@Rimsilver}{0.000}
\@namedef{r@WT@Rimstrict}{0.333}
\@namedef{r@WT@Rlow}{0.212}
\@namedef{r@WT@RlowHi}{0.481}
\@namedef{r@WT@RlowLo}{0.000}
\@namedef{r@WT@Rlown}{2.3}
\@namedef{r@WT@Rst}{0.563}
\@namedef{r@WT@Seeds}{3}
\@namedef{r@WT@bmlexF1}{0.412}
\@namedef{r@WT@bmlexRim}{0.208}
\@namedef{r@WT@bmpred}{1.07}
\@namedef{r@WTD@AdjMax}{0.398}
\@namedef{r@WTD@AdjMin}{0.319}
\@namedef{r@WTD@F1}{0.350}
\@namedef{r@WTD@Fadjudicated}{0.348}
\@namedef{r@WTD@Fhi}{0.500}
\@namedef{r@WTD@Flenient}{0.378}
\@namedef{r@WTD@Flinked}{0.428}
\@namedef{r@WTD@Flo}{0.242}
\@namedef{r@WTD@Fmain}{0.350}
\@namedef{r@WTD@Fnolink}{0.140}
\@namedef{r@WTD@Fnopred}{0.329}
\@namedef{r@WTD@Fsilver}{0.319}
\@namedef{r@WTD@Fstrict}{0.337}
\@namedef{r@WTD@P}{0.257}
\@namedef{r@WTD@Pred}{2.27}
\@namedef{r@WTD@R}{0.563}
\@namedef{r@WTD@Rhigh}{0.627}
\@namedef{r@WTD@Rim}{0.312}
\@namedef{r@WTD@Rimadjudicated}{0.317}
\@namedef{r@WTD@Rimlenient}{0.312}
\@namedef{r@WTD@Rimlo}{0.286}
\@namedef{r@WTD@Rimmain}{0.312}
\@namedef{r@WTD@Rimnopred}{0.312}
\@namedef{r@WTD@Rimsilver}{0.000}
\@namedef{r@WTD@Rimstrict}{0.312}
\@namedef{r@WTD@Rlow}{0.273}
\@namedef{r@WTD@RlowHi}{0.571}
\@namedef{r@WTD@RlowLo}{0.000}
\@namedef{r@WTD@Rlown}{3.0}
\@namedef{r@WTD@Rst}{0.690}
\@namedef{r@WTD@Seeds}{3}
\@namedef{r@WTD@bmlexF1}{0.359}
\@namedef{r@WTD@bmlexRim}{0.479}
\@namedef{r@WTD@bmpred}{2.39}
\@namedef{r@ZTDR@AdjMax}{0.825}
\@namedef{r@ZTDR@AdjMin}{0.700}
\@namedef{r@ZTDR@F1}{0.799}
\@namedef{r@ZTDR@Fadjudicated}{0.749}
\@namedef{r@ZTDR@Fhi}{0.885}
\@namedef{r@ZTDR@Flenient}{0.777}
\@namedef{r@ZTDR@Flinked}{0.834}
\@namedef{r@ZTDR@Flo}{0.702}
\@namedef{r@ZTDR@Fmain}{0.799}
\@namedef{r@ZTDR@Fnolink}{0.675}
\@namedef{r@ZTDR@Fnopred}{0.787}
\@namedef{r@ZTDR@Fsilver}{0.568}
\@namedef{r@ZTDR@Fstrict}{0.745}
\@namedef{r@ZTDR@P}{0.738}
\@namedef{r@ZTDR@Pred}{1.21}
\@namedef{r@ZTDR@R}{0.874}
\@namedef{r@ZTDR@Rhigh}{0.887}
\@namedef{r@ZTDR@Rim}{0.896}
\@namedef{r@ZTDR@Rimadjudicated}{0.810}
\@namedef{r@ZTDR@Rimlenient}{0.896}
\@namedef{r@ZTDR@Rimlo}{0.810}
\@namedef{r@ZTDR@Rimmain}{0.896}
\@namedef{r@ZTDR@Rimnopred}{0.896}
\@namedef{r@ZTDR@Rimsilver}{0.000}
\@namedef{r@ZTDR@Rimstrict}{0.896}
\@namedef{r@ZTDR@Rlow}{0.818}
\@namedef{r@ZTDR@RlowHi}{1.000}
\@namedef{r@ZTDR@RlowLo}{0.600}
\@namedef{r@ZTDR@Rlown}{9.0}
\@namedef{r@ZTDR@Rst}{0.857}
\@namedef{r@ZTDR@Seeds}{3}
\@namedef{r@ZTR@AdjMax}{0.762}
\@namedef{r@ZTR@AdjMin}{0.637}
\@namedef{r@ZTR@F1}{0.724}
\@namedef{r@ZTR@Fadjudicated}{0.696}
\@namedef{r@ZTR@Fhi}{0.801}
\@namedef{r@ZTR@Flenient}{0.725}
\@namedef{r@ZTR@Flinked}{0.768}
\@namedef{r@ZTR@Flo}{0.636}
\@namedef{r@ZTR@Fmain}{0.724}
\@namedef{r@ZTR@Fnolink}{0.582}
\@namedef{r@ZTR@Fnopred}{0.707}
\@namedef{r@ZTR@Fsilver}{0.520}
\@namedef{r@ZTR@Fstrict}{0.671}
\@namedef{r@ZTR@P}{0.643}
\@namedef{r@ZTR@Pred}{1.32}
\@namedef{r@ZTR@R}{0.831}
\@namedef{r@ZTR@Rhigh}{0.820}
\@namedef{r@ZTR@Rim}{0.833}
\@namedef{r@ZTR@Rimadjudicated}{0.810}
\@namedef{r@ZTR@Rimlenient}{0.833}
\@namedef{r@ZTR@Rimlo}{0.810}
\@namedef{r@ZTR@Rimmain}{0.833}
\@namedef{r@ZTR@Rimnopred}{0.833}
\@namedef{r@ZTR@Rimsilver}{0.000}
\@namedef{r@ZTR@Rimstrict}{0.833}
\@namedef{r@ZTR@Rlow}{0.879}
\@namedef{r@ZTR@RlowHi}{1.000}
\@namedef{r@ZTR@RlowLo}{0.727}
\@namedef{r@ZTR@Rlown}{9.7}
\@namedef{r@ZTR@Rst}{0.849}
\@namedef{r@ZTR@Seeds}{3}
\@namedef{r@all@belowDiag}{17}
\@namedef{r@all@belowDiagOv}{16}
\@namedef{r@all@gainLLM}{0.271}
\@namedef{r@all@gainLex}{0.188}
\@namedef{r@all@gainShare}{69\%}
\@namedef{r@all@gapOver}{14}
\@namedef{r@all@invalidAll}{18}
\@namedef{r@all@invalidWT}{4}
\@namedef{r@all@maxBaseAdj}{0.508}
\@namedef{r@all@maxSeeds}{3}
\@namedef{r@all@maxSmallAdj}{0.621}
\@namedef{r@all@minSeeds}{3}
\@namedef{r@all@nHigh}{50}
\@namedef{r@all@nImLo}{7}
\@namedef{r@all@nLLM}{18}
\@namedef{r@all@nLow}{11}
\@namedef{r@all@nSys}{20}
\@namedef{r@all@parseErr}{51}
\@namedef{r@c1@absdiff}{0.050}
\@namedef{r@c1@diff}{+0.050}
\@namedef{r@c1@hi}{+0.127}
\@namedef{r@c1@lo}{-0.027}
\@namedef{r@c1@p}{0.215}
\@namedef{r@c1@pholm}{0.645}
\@namedef{r@c2@absdiff}{0.006}
\@namedef{r@c2@diff}{$-$0.006}
\@namedef{r@c2@hi}{+0.076}
\@namedef{r@c2@lo}{-0.081}
\@namedef{r@c2@p}{0.898}
\@namedef{r@c2@pholm}{0.898}
\@namedef{r@c3@absdiff}{0.040}
\@namedef{r@c3@diff}{$-$0.040}
\@namedef{r@c3@hi}{+0.040}
\@namedef{r@c3@lo}{-0.132}
\@namedef{r@c3@p}{0.324}
\@namedef{r@c3@pholm}{0.648}
\@namedef{r@c4@absdiff}{0.120}
\@namedef{r@c4@diff}{+0.120}
\@namedef{r@c4@hi}{+0.247}
\@namedef{r@c4@lo}{+0.004}
\@namedef{r@c4@p}{0.043}
\@namedef{r@c4@pholm}{0.215}
\@namedef{r@c5@absdiff}{0.321}
\@namedef{r@c5@diff}{+0.321}
\@namedef{r@c5@hi}{+0.425}
\@namedef{r@c5@lo}{+0.214}
\@namedef{r@c5@p}{<0.001}
\@namedef{r@c5@pholm}{0.005}
\@namedef{r@c6@absdiff}{0.151}
\@namedef{r@c6@diff}{+0.151}
\@namedef{r@c6@hi}{+0.246}
\@namedef{r@c6@lo}{+0.061}
\@namedef{r@c6@p}{0.001}
\@namedef{r@c6@pholm}{0.008}
\@namedef{r@c7@absdiff}{0.126}
\@namedef{r@c7@diff}{+0.126}
\@namedef{r@c7@hi}{+0.204}
\@namedef{r@c7@lo}{+0.055}
\@namedef{r@c7@p}{0.001}
\@namedef{r@c7@pholm}{0.008}
\@namedef{r@c8@absdiff}{0.271}
\@namedef{r@c8@diff}{+0.271}
\@namedef{r@c8@hi}{+0.439}
\@namedef{r@c8@lo}{+0.095}
\@namedef{r@c8@p}{0.011}
\@namedef{r@c8@pholm}{0.066}
\@namedef{r@c9@absdiff}{0.208}
\@namedef{r@c9@diff}{+0.208}
\@namedef{r@c9@hi}{+0.375}
\@namedef{r@c9@lo}{+0.000}
\@namedef{r@c9@p}{0.052}
\@namedef{r@c9@pholm}{0.215}
\@namedef{r@p1@absdiff}{0.290}
\@namedef{r@p1@diff}{+0.290}
\@namedef{r@p1@hi}{+0.430}
\@namedef{r@p1@lo}{+0.172}
\@namedef{r@p1@p}{<0.001}
\@namedef{r@p2@absdiff}{0.040}
\@namedef{r@p2@diff}{+0.040}
\@namedef{r@p2@hi}{+0.101}
\@namedef{r@p2@lo}{-0.025}
\@namedef{r@p2@p}{0.219}
\@namedef{r@p3@absdiff}{0.023}
\@namedef{r@p3@diff}{$-$0.023}
\@namedef{r@p3@hi}{+0.033}
\@namedef{r@p3@lo}{-0.072}
\@namedef{r@p3@p}{0.376}
\@namedef{r@p4@absdiff}{0.004}
\@namedef{r@p4@diff}{$-$0.004}
\@namedef{r@p4@hi}{+0.036}
\@namedef{r@p4@lo}{-0.043}
\@namedef{r@p4@p}{0.796}
\@namedef{r@p5@absdiff}{0.043}
\@namedef{r@p5@diff}{+0.043}
\@namedef{r@p5@hi}{+0.119}
\@namedef{r@p5@lo}{-0.037}
\@namedef{r@p5@p}{0.285}
\@namedef{r@p6@absdiff}{0.042}
\@namedef{r@p6@diff}{+0.042}
\@namedef{r@p6@hi}{+0.115}
\@namedef{r@p6@lo}{-0.028}
\@namedef{r@p6@p}{0.254}
\@namedef{r@p7@absdiff}{0.079}
\@namedef{r@p7@diff}{+0.079}
\@namedef{r@p7@hi}{+0.155}
\@namedef{r@p7@lo}{+0.013}
\@namedef{r@p7@p}{0.027}
\makeatother

